Public Domain Rank: Identifying Notable Individuals with the Wisdom of the Crowd

Identifying literary, scientific, and technical works of enduring interest is challenging. Few are able to name significant works across more than a handful of domains or languages. This paper introduces an automatic method for identifying authors of notable works throughout history. Notability is defined using the record of which works volunteers have made available in public domain digital editions. A significant benefit of this bottom-up approach is that it also provides a novel and reproducible index of notability for all individuals with Wikipedia pages. The method promises to supplement the work of cultural organizations and institutions seeking to publicize the availability of notable works and prioritize works for preservation and digitization.

==> tables/ranking-1970s.tex <==
\begin{table}
\footnotesize\begin{tabular}{lrrr}
\toprule
                      &     \ding{61} &  Views & Public Domain Rank (Score) \\
\midrule
                      &       &        &                            \\
       Leigh Brackett &  1978 &     63 &                   245 (95) \\
       August Derleth &  1971 &     77 &                   342 (95) \\
      Edmond Hamilton &  1977 &     27 &                   365 (95) \\
        Fredric Brown &  1972 &     69 &                   442 (94) \\
        Bruce Elliott &  1973 &      3 &                   456 (94) \\
  Miriam Allen deFord &  1975 &      4 &                   467 (94) \\
      Alice Dalgliesh &  1979 &      5 &                   488 (94) \\
     J. R. R. Tolkien &  1973 &   4634 &                   733 (94) \\
       Edgar Pangborn &  1976 &      9 &                   810 (94) \\
   Eric Frank Russell &  1978 &     24 &                   829 (94) \\
        Jean Stafford &  1979 &     17 &                  1076 (94) \\
     John W. Campbell &  1971 &     80 &                  1099 (94) \\
          Ruth Sawyer &  1970 &      6 &                  1281 (94) \\
 Amelia Reynolds Long &  1978 &      1 &                  1370 (94) \\
          W. H. Auden &  1973 &    615 &                  1638 (94) \\
          Kate Seredy &  1975 &      7 &                  1701 (94) \\
      Agatha Christie &  1976 &   2043 &                  1770 (94) \\
     Vincent Starrett &  1974 &      6 &                  1784 (94) \\
         Philip Wylie &  1971 &     28 &                  1800 (94) \\
    Charles R. Tanner &  1974 &      3 &                  1885 (94) \\
\bottomrule
\end{tabular}

\caption{Public Domain Rank and Score for individuals who died between 1970 and 1979.}\label{ranking-1970s}
\end{table}

==> tables/rankings-american-singers.tex <==
\begin{table}
\footnotesize\begin{tabular}{lrrr}
\toprule
                          &     \ding{61} &  Views & Public Domain Rank (Score) \\
\midrule
                          &       &        &                            \\
         Sammy Davis, Jr. &  1990 &   1345 &                 17948 (91) \\
                 Liberace &  1987 &   3669 &                 19087 (91) \\
        Annette Funicello &  2013 &   1728 &                 24876 (90) \\
             Ethel Merman &  1984 &    355 &                 29111 (90) \\
            Dick Van Dyke &   NA &   2029 &                 29733 (90) \\
           Marilyn Monroe &  1962 &   9886 &                 29968 (90) \\
        Weird Al Yankovic &   NA &    271 &                 32382 (89) \\
             Vic Mignogna &   NA &    460 &                 35376 (89) \\
           Frankie Avalon &   NA &    616 &                 36148 (89) \\
 Floyd Red Crow Westerman &  2007 &     82 &                 37976 (89) \\
              Mary Martin &  1990 &    231 &                 38378 (89) \\
              Dean Martin &  1995 &   1894 &                 38575 (89) \\
               Dana Reeve &  2006 &    393 &                 40070 (88) \\
               Lance Bass &   NA &   1090 &                 41305 (88) \\
              Jodi Benson &   NA &    457 &                 41816 (88) \\
            Elvis Presley &  1977 &   7796 &                 42823 (88) \\
              Keith Andes &  2005 &     55 &                 43676 (88) \\
                Ken Berry &   NA &    258 &                 45429 (88) \\
             Jim Morrison &  1971 &   3042 &                 46255 (88) \\
          Louis Armstrong &  1971 &   2182 &                 50474 (87) \\
\bottomrule
\end{tabular}

\caption{Ranking of 20th century American singers.}\label{rankings-american-singers}
\end{table}

==> tables/rankings-popular-literary.tex <==
\begin{table}
\footnotesize\begin{tabular}{lrrr}
\toprule
                    &     \ding{61} &  Views & Public Domain Rank (Score) \\
\midrule
                    &       &        &                            \\
 Zora Neale Hurston &  1960 &    448 &                  3056 (94) \\
       Iris Murdoch &  1999 &    244 &                  3362 (94) \\
     Danielle Steel &   NA &    496 &                  5524 (93) \\
        P. D. James &   NA &    271 &                  5807 (93) \\
      Stieg Larsson &  2004 &    811 &                 53698 (87) \\
\bottomrule
\end{tabular}

\caption{Rankings of selected writers of "popular" and "literary" prose fiction.}\label{rankings-popular-literary}
\end{table}
